Black Hole Phenomenology and Dark Matter Searches

Motivated by recent detections of black hole binary systems through gravitational waves, in this thesis we discuss two complementary channels for the observation of Primordial Black Holes (PBHs) with masses between a few and a hundred solar masses. First, we consider the possibility of detecting black holes in the Milky Way through the electromagnetic radiation emitted in the process of gas accretion, separately examining the astrophysical black hole population and an hypothetical primordial one. We employ a state-of-the-art accretion model, able to account for radiative feedback. Our findings suggest that the detection of astrophysical isolated black holes in the vicinity of the galactic center is around the corner. We perform a complete parametric study of the uncertainty associated with this prediction. We then turn to constraining PBH abundance through the same channel, finding that existing bounds can be significantly relaxed when modelling uncertainties are taken into account. The PBH mass function motivated by the Universe's thermal history is considered. In the second part, we turn to gravitational wave observations. The possibility of disentangling the astrophysical background form a possible primordial signal in present data is hampered by large theoretical uncertainties on the properties of both populations. However, third-generation gravitational wave detectors will be able to detect mergers up to the dark ages, where the astrophysical background is expected to be absent. Through mock data generation and analysis, we assess the ability of the Einstein Telescope (ET) to identify a subdominant population of PBHs, disentangling it from the astrophysical one based exclusively on event distance measurements. We find that the ET should be able to detect and constrain the PBH abundance if these constitute at least approximately one part in $10^5$ of the dark matter.

==> content/colophon.tex <==
% !TEX root = ../my-thesis.tex
%
\pagestyle{empty}
\hfill
\vfill
\pdfbookmark[0]{Colophon}{Colophon}
\section*{Colophon}

This thesis was typeset with \LaTeXe.
It uses the \textit{Clean Thesis} style developed by Ricardo Langner.
The design of the \textit{Clean Thesis} style is inspired by user guide documents from Apple Inc.

Download the \textit{Clean Thesis} style at \url{http://cleanthesis.der-ric.de/}.


==> content/declaration.tex <==
% !TEX root = ../my-thesis.tex
%
%************************************************
% Declaration
%************************************************
\pdfbookmark[0]{Declaration}{Declaration}
\addchap{Declaration}
\label{sec:declaration}
\thispagestyle{empty}

You can put your declaration here, to declare that you have completed your work solely and only with the help of the references you mentioned.

\bigskip

\noindent\textit{\thesisUniversityCity, \thesisDate}

\smallskip

\begin{flushright}
	\begin{minipage}{5cm}
		\rule{\textwidth}{1pt}
		\centering\thesisName
	\end{minipage}
\end{flushright}

%*****************************************
%*****************************************


==> content/titlepages.tex <==
% !TEX root = ../my-thesis.tex
%
% ------------------------------------  --> cover title page
\begin{titlepage}
	\pdfbookmark[0]{Cover}{Cover}
	\flushright
	\hfill
	\vfill
	{\LARGE\thesisTitle \par}
	\rule[5pt]{\textwidth}{.4pt} \par
	{\Large\thesisName}
	\vfill
	%\textit{\large\thesisDate} \\
	%Version: \thesisVersion
\end{titlepage}


% ------------------------------------  --> main title page
%\begin{titlepage}
%	\pdfbookmark[0]{Titlepage}{Titlepage}
%	\tgherosfont
%	\centering

%	{\Large \thesisUniversity} \\[4mm]
%	\includegraphics[width=6cm]{gfx/Clean-Thesis-Logo} \\[2mm]
	%\textsf{\thesisUniversityDepartment} \\
%	\textsf{\thesisUniversityInstitute} \\
	%\textsf{\thesisUniversityGroup} \\

%	\vfill
	%{\large \thesisSubject} \\[5mm]
%	{\LARGE \color{ctcolortitle}\textbf{\thesisTitle} \\[10mm]}
%	{\Large \thesisName} \\

%	\vfill
%	\begin{minipage}[t]{.27\textwidth}
	%	\raggedleft
	%	\textit{1. Reviewer}
	%\end{minipage}
%	\hspace*{15pt}
%	\begin{minipage}[t]{.65\textwidth}
%		{\Large \thesisFirstReviewer} \\
%	  	{\small \thesisFirstReviewerDepartment} \\[-1mm]
%		{\small \thesisFirstReviewerUniversity}
%	\end{minipage} \\[5mm]
%	\begin{minipage}[t]{.27\textwidth}
	%	\raggedleft
	%	\textit{2. Reviewer}
%	\end{minipage}
%	\hspace*{15pt}
%	\begin{minipage}[t]{.65\textwidth}
	%	{\Large \thesisSecondReviewer} \\
	  %	{\small \thesisSecondReviewerDepartment} \\[-1mm]
%		{\small \thesisSecondReviewerUniversity}
%	\end{minipage} \\[10mm]
%	\begin{minipage}[t]{.27\textwidth}
	%	\raggedleft
	%	\textit{Supervisors}
%	\end{minipage}
%	\hspace*{15pt}
%	\begin{minipage}[t]{.65\textwidth}
%		\thesisFirstSupervisor\ and \thesisSecondSupervisor
%	\end{minipage} \\[10mm]

%	\thesisDate \\

%\end{titlepage}




